ICDAR 2021 Competition on Document VisualQuestion Answering

In this report we present results of the ICDAR 2021 edition of the Document Visual Question Challenges. This edition complements the previous tasks on Single Document VQA and Document Collection VQA with a newly introduced on Infographics VQA. Infographics VQA is based on a new dataset of more than 5,000 infographics images and 30,000 question-answer pairs. The winner methods have scored 0.6120 ANLS in Infographics VQA task, 0.7743 ANLSL in Document Collection VQA task and 0.8705 ANLS in Single Document VQA. We present a summary of the datasets used for each task, description of each of the submitted methods and the results and analysis of their performance. A summary of the progress made on Single Document VQA since the first edition of the DocVQA 2020 challenge is also presented.

==> figures/t3_anls_by_types.tex <==


\begin{figure}[!ht]
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{images/plots/T3_Answer types.png}
  \label{fig:anls_by_answer_type}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{images/plots/T3_Evidence types.png}
  \label{fig:anls_by_evidence_type}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=\linewidth]{images/plots/T3_Operation types.png}
  \label{fig:anls_by_operation_type}
\endminipage
\caption{ANLS by answer type (left), by evidence type (center) and operation (right).}
\end{figure}

==> figures/t3_ansls_by_types_2.tex <==
\begin{figure}[hp]
    \centering
    \begin{subfigure}[t]{1\textwidth}
        \centering
        \includegraphics[width=\linewidth, height=5cm]{images/infovqa_qt.pdf}
        % \caption{question type}
        \label{fig:infovqa_question_types_results}
    \end{subfigure}
    
    \begin{subfigure}{1\textwidth}
        \centering
        \includegraphics[width=\linewidth, height=5cm]{images/infovqa_et.pdf}
        % \caption{evidence type}
        \label{fig:infovqa_evidence_types_results}
    \end{subfigure}
    
    \begin{subfigure}[b]{1\textwidth}
        \centering
        \includegraphics[width=\linewidth, height=5cm]{images/infovqa_ot.pdf}
        % \caption{operation type}
        \label{fig:infovqa_operation_types_results}
    \end{subfigure}
    \vspace{-10.0mm}
    \caption{\textbf{ANLS score of InfographicVQA task methods} breakdown by answer types (top), evidence type (middle) and operations required to answer the posed questions (bottom).}
    \label{fig:infovqa_breakdown}
\end{figure}


==> figures/three_tasks_samples.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/three_tasks_challenge_report.png}
    \caption{Examples for the three different tasks in DocVQA. \TaskA task is a standard VQA on business/industry documents. Instead, in \TaskB task, questions are asked on a document collection comprising documents of same template. Finally, \TaskC task is similar to \TaskA task, but the images in the dataset are infographics.}
    \label{fig:three_taks_examples}
\end{figure*}

==> tables/task1_results_old.tex <==
\setlength{\tabcolsep}{8pt}  % Increase the separation space between columns.

\begin{table}[ht]
\centering
\begin{tabular}{lr}
\toprule
Method          & \multicolumn{1}{c}{ANLS} \\
\midrule
Applica.ai TILT                & \textbf{0.8705} \\
LayoutLM 2.0 (single model)    & 0.8672 \\
Alibaba DAMO NLP               & 0.8506 \\
PingAn-OneConnect-Gammalab-DQA & 0.8484 \\
Structural LM-v2               & 0.7674 \\
QA\_Base\_MRC\_2               & 0.7415 \\
QA\_Base\_MRC\_1               & 0.7407 \\
HyperDQA\_V4                   & 0.6893 \\
UGLIFT v0.1 (Clova OCR)        & 0.4417 \\
Plain BERT QA                  & 0.3524 \\
HDNet                          & 0.3401 \\
CLOVA OCR                      & 0.3296 \\
docVQAQV\_V0.1                 & 0.3016 \\
\bottomrule
\end{tabular}
\vspace{2mm}
\caption{\textbf{\TaskA task results table.}}

\label{tab:task1_results}
\end{table}

\setlength{\tabcolsep}{6pt}  % Restore column separation to its default value.

==> tables/task1_results_old_old.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lr}
\toprule
Method          & \multicolumn{1}{c}{ANLS} \\
\midrule
Applica.ai TILT                & \textbf{0.8705} \\
LayoutLM 2.0 (single model)    & 0.8672 \\
Alibaba DAMO NLP               & 0.8506 \\
QA\_Base\_MRC\_2               & 0.7415 \\
UGLIFT v0.1 (Clova OCR)        & 0.4417 \\
\midrule
PingAn-OneConnect-Gammalab-DQA & 0.8484 \\
Structural LM-v2               & 0.7674 \\
QA\_Base\_MRC\_1               & 0.7407 \\
HyperDQA\_V4                   & 0.6893 \\
Plain BERT QA                  & 0.3524 \\
HDNet                          & 0.3401 \\
CLOVA OCR                      & 0.3296 \\
docVQAQV\_V0.1                 & 0.3016 \\
\bottomrule
\end{tabular}
\vspace{2mm}
\caption{\textbf{\TaskA task results table.} Top section shows methods within the ICDAR 2021 edition. Bottom section shows methods from previous CVPR 2020 edition~\cite{docvqa_das}.}
\label{tab:task1_results}
\end{table}

==> tables/task2_results_old.tex <==
\setlength{\tabcolsep}{8pt}  % Increase the separation space between columns.

\begin{table}[hb]
\centering
\begin{tabular}{lrr}
\toprule
Method       & \begin{tabular}[c]{@{}c@{}}Answering\\ ANLSL\end{tabular} & \begin{tabular}[c]{@{}c@{}}Retrieval\\ MAP\end{tabular} \\
\midrule
\infrarrd                                   & \textbf{0.7743}   & 74.66\% \\
(Baseline) Database~\cite{doccvqa_icdar}               & 0.7068            & 71.06\% \\
(Baseline) TS-BERT~\cite{doccvqa_icdar}     & 0.4513	        & 72.84\% \\
DQA~\cite{docvqa_das}                       & 0.0000            & \textbf{80.90}\% \\
DOCR~\cite{docvqa_das}                      & 0.0000            & 79.15\% \\
\bottomrule
\end{tabular}
\vspace{1.5mm}
\caption{\textbf{\TaskB task results table.}}
\label{tab:task2_results}
\end{table}

\setlength{\tabcolsep}{6pt}  % Restore column separation to its default value.

==> tables/task2_results_old_old.tex <==
\setlength{\tabcolsep}{8pt}  % Increase the separation space between columns.

\begin{table}[hb]
\centering
\begin{tabular}{lrr}
\toprule
Method       & \begin{tabular}[c]{@{}c@{}}Answering\\ ANLSL\end{tabular} & \begin{tabular}[c]{@{}c@{}}Retrieval\\ MAP\end{tabular} \\
\midrule
\infrarrd                                   & \textbf{0.7743}   & 74.66\% \\
\midrule
Database~\cite{doccvqa_icdar}               & 0.7068            & 71.06\% \\
Text spotting-BERT~\cite{doccvqa_icdar}     & 0.4513	        & 72.84\% \\
\midrule
DQA~\cite{docvqa_das}                       & 0.0000            & \textbf{80.90}\% \\
DOCR~\cite{docvqa_das}                      & 0.0000            & 79.15\% \\
\bottomrule
\end{tabular}
\vspace{1.5mm}
\caption[hello]{\textbf{\TaskB task results table.} Top section show methods within the ICDAR 2021 edition. Middle section shows baseline methods results proposed by the competition organizers~\cite{doccvqa_icdar}. Bottom section show methods from previous CVPR 2020 edition~\cite{docvqa_das}.}
\label{tab:task2_results}
\end{table}

\setlength{\tabcolsep}{6pt}  % Restore column separation to its default value.

==> tables/task3_results_old.tex <==
\begin{table}[hb]
\centering
\begin{tabular}{lr}
\toprule
Method          & \multicolumn{1}{c}{ANLS} \\
\midrule
\tilt           & \textbf{0.6120}         \\
\igbert         & 0.3854                  \\
\clova          & 0.3219                  \\
\ensemble       & 0.2853                  \\
\bertba         & 0.2078                  \\
\bert           & 0.1678                  \\        
\midrule
Human           & 0.980                   \\
\layoutlm       & 0.272                   \\
\mc             & 0.147                   \\
\bottomrule
\end{tabular}
\vspace{2mm}
\caption{\textbf{\TaskC task results table.} Top section show methods withing the ICDAR 2021 competition. Bottom section shows baseline methods proposed by the competition organizers.}
\label{tab:task3_results}
\end{table}
